Estimating Uncertainty Online Against an Adversary

Assessing uncertainty is an important step towards ensuring the safety and reliability of machine learning systems. Existing uncertainty estimation techniques may fail when their modeling assumptions are not met, e.g. when the data distribution differs from the one seen at training time. Here, we propose techniques that assess a classification algorithm's uncertainty via calibrated probabilities (i.e. probabilities that match empirical outcome frequencies in the long run) and which are guaranteed to be reliable (i.e. accurate and calibrated) on out-of-distribution input, including input generated by an adversary. This represents an extension of classical online learning that handles uncertainty in addition to guaranteeing accuracy under adversarial assumptions. We establish formal guarantees for our methods, and we validate them on two real-world problems: question answering and medical diagnosis from genomic data.

==> figures/Makefile <==
LATEX = pdflatex
#LATEX = pdflatex -interaction=nonstopmode
FIGURES = $(wildcard *.tikz)
PDFS = $(patsubst %.tikz,%.pdf,$(FIGURES))

all:
	make synth.pdf
	make semparse.pdf
	make wtccc.pdf

# all: $(PDFS)

# %.pdf: %.tikz
# 	$(LATEX) $<

clean:
	rm -rf *.{aux,bbl,blg,log,out}
	rm -rf $(OUTPUT).pdf

.PHONY: clean bib final

semparse.pdf: data
	python ./calibration-plots.py \
	  --cal data/semparse-cal.txt \
	  --hist data/semparse-hist.txt \
	  --metrics data/semparse-metrics.txt \
	  --plots data/semparse-plots.txt \
	  --out $@

wtccc.pdf: data
	python ./calibration-plots.py \
	  --cal data/wtccc-cal.txt \
	  --hist data/wtccc-hist.txt \
	  --metrics data/wtccc-metrics.txt \
	  --plots data/wtccc-plots.txt \
	  --out $@

synth.pdf: data
	python ./synth-calibration-plots.py \
	  --bernoulli-plots ./data/synthetic-bernoulli.txt \
	  --adversarial-plots ./data/synthetic-adversarial.txt \
	  --out $@


==> figures/data/Makefile <==
SCRIPTS:=../scripts
DATA:=../data
TARGET:=../../doc/aistats2016/figures/data

all:
	make semparse
	make wtccc
	make synthetic-bernoulli.txt
	make synthetic-adversarial.txt
	make copy

copy:
	cp ./*.txt $(TARGET)

semparse:
	echo $(PYTHONPATH)
	python $(SCRIPTS)/gen-semparse.py \
	  --val $(DATA)/semparse/train.log \
	  --test $(DATA)/semparse/test.log \
	  --out-cal ./semparse-cal.txt \
	  --out-hist ./semparse-hist.txt \
	  --out-metrics ./semparse-metrics.txt \
	  --out-plots ./semparse-plots.txt
	touch $@

wtccc:
	python $(SCRIPTS)/gen-wtccc.py \
	  --cases $(DATA)/wtccc/T1D.top.sorted.input \
	  --controls $(DATA)/wtccc/58C.top.sorted.input \
	  --out-cal ./wtccc-cal.txt \
	  --out-hist ./wtccc-hist.txt \
	  --out-metrics ./wtccc-metrics.txt \
	  --out-plots ./wtccc-plots.txt
	touch $@

synthetic-bernoulli.txt:
	python $(SCRIPTS)/recalibration-bernoulli.py --out-plots $@

synthetic-adversarial.txt:
	python $(SCRIPTS)/recalibration-adversarial.py --out-plots $@

